Local Supports Global: Deep Camera Relocalization with Sequence Enhancement

We propose to leverage the local information in image sequences to support global camera relocalization. In contrast to previous methods that regress global poses from single images, we exploit the spatial-temporal consistency in sequential images to alleviate uncertainty due to visual ambiguities by incorporating a visual odometry (VO) component. Specifically, we introduce two effective steps called content-augmented pose estimation and motion-based refinement. The content-augmentation step focuses on alleviating the uncertainty of pose estimation by augmenting the observation based on the co-visibility in local maps built by the VO stream. Besides, the motion-based refinement is formulated as a pose graph, where the camera poses are further optimized by adopting relative poses provided by the VO component as additional motion constraints. Thus, the global consistency can be guaranteed. Experiments on the public indoor 7-Scenes and outdoor Oxford RobotCar benchmark datasets demonstrate that benefited from local information inherent in the sequence, our approach outperforms state-of-the-art methods, especially in some challenging cases, e.g., insufficient texture, highly repetitive textures, similar appearances, and over-exposure.

==> Sections/Abstract-20190313.tex <==
\begin{abstract}
	%Visual localization plays a key role in various computer vision tasks including robotics and virtual/augmented reality. With the advent of convolutional neural networks (CNNs), a plethora of algorithms have been proposed to estimate global poses from a single image in an end-to-end fashion. 
	We present a novel architecture to learn camera relocalization from video clips by incorporating a visual odometry (VO) component. In contrast to most previous methods regressing the global pose with high uncertainty from a single image, we propose to reduce such uncertainty by considering the spatio-temporal consistency in sequential images. In specific, we introduce two effective steps called content-augmented pose estimation and motion-based refinement. The content-augmentation step focuses on alleviating the uncertainty of pose estimation by augmenting the observation based on the co-visibility in the local map. Besides, the camera poses are further improved by adopting VO results as constraints to enforce global consistency. With the global and relative poses representing notes and edges respectively, global poses are optimized within a pose graph during training and testing processes. Experiments on the public indoor 7-Scenes and outdoor Oxford RobotCar benchmark datasets demonstrate our approach outperforms previous methods consistently. Especially, our model achieves outstanding performance in challenging conditions e.g. texture-less regions, over-exposure, where prior methods tend to produce poor performance.
	% 	estimating the global pose from a single image suffers from high uncertainty. In contrast, we propose to learn camera localization and visual odometry jointly from video clips in a unified architecture. Instead of tackling the problem with brute force,
	
\end{abstract}


==> Sections/Abstract-20190322.tex <==
\begin{abstract}
	%Visual localization plays a key role in various computer vision tasks including robotics and virtual/augmented reality. With the advent of convolutional neural networks (CNNs), a plethora of algorithms have been proposed to estimate global poses from a single image in an end-to-end fashion. 
	We propose to leverage the local information in videos to support global camera relocalization. In contrast to most previous methods regressing the global poses with high uncertainties from single images, we reduce such uncertainty exploiting the spatio-temporal consistency in sequential images by incorporating a VO component. Specifically, we introduce two effective steps called content-augmented pose estimation and motion-based refinement. The content-augmentation step focuses on alleviating the uncertainty of pose estimation by augmenting the observation based on the co-visibility in the local map. Besides, the camera poses are further improved by adopting VO results as constraints to enforce global consistency. With the global and relative poses representing notes and edges respectively, global poses are optimized within a pose graph during training and testing processes. Experiments on the public indoor 7-Scenes and outdoor Oxford RobotCar benchmark datasets demonstrate our approach outperforms previous methods consistently. Especially, our model achieves outstanding performance in challenging conditions e.g. texture-less regions, highly repetitve textures, over-exposure, where prior methods tend to produce poor performance.
	% 	estimating the global pose from a single image suffers from high uncertainty. In contrast, we propose to learn camera localization and visual odometry jointly from video clips in a unified architecture. Instead of tackling the problem with brute force,
	
\end{abstract}


==> Sections/Abstract.tex <==
\begin{abstract}
	%Visual localization plays a key role in various computer vision tasks including robotics and virtual/augmented reality. With the advent of convolutional neural networks (CNNs), a plethora of algorithms have been proposed to estimate global poses from a single image in an end-to-end fashion. 
	We present a novel architecture to learn camera relocalization and visual odometry jointly from video clips in a unified model. In contrast to most previous methods regressing the global pose with high uncertainty from a single image due to the noise, repetitive textures, over-exposure, et al., we propose to reduce such uncertainty by taking advantages of the spatio-temporal consistency provided by sequential images. In specific, we delve into the nature of videos by introducing two effective steps called \textit{content-} and \textit{motion-based} refinement. The \textit{content-based} step focuses on alleviating the uncertainty of estimated poses by augmenting the observation based on the co-visibility over sequential images. Besides, VO produces accurate relative poses but undergoes error accumulation while re-localization suffers from pose uncertainty but is drift-free. Leveraging the motion characteristics of the two sub-tasks, results of re-localization and VO estimation are further improved by enforcing global motion consistency employing a pose graph optimization. Experiments on the public indoor 7-Scenes and outdoor Oxford RobotCar benchmark datasets demonstrate our approach outperforms previous methods consistently. Especially, our model achieves outstanding performance in challenging conditions such as texture-less regions, over-exposure, et al., where prior methods tend to produce poor performance.
	% 	estimating the global pose from a single image suffers from high uncertainty. In contrast, we propose to learn camera localization and visual odometry jointly from video clips in a unified architecture. Instead of tackling the problem with brute force,
	
\end{abstract}


==> Sections/Conclusion.tex <==
\section{Introduction}


==> Sections/Introduction-20190313.tex <==
\section{Introduction}
\label{introduction}

%The problem of identifying the position of the camera that captured an image of a scene has been studied extensively for decades [34, 33, 4]. With applications in domains such as robotics and autonomous driving, a considerable amount of engineering effort has been dedicated to developing systems for different versions of the problem. One formulation, often referred to as simply ‘localization’, assumes that a map of the 3D scene is provided in advance and the goal is to localize any new image of the scene relative to this map. A second formulation, commonly referred to as ‘Simultaneous Localization and Mapping’ (SLAM), assumes that there is no prespecified map of the scene, and that it should be estimated concurrently with the locations of each observed image. Research on this topic has focused on different aspects and challenges including: estimating the displacement between frames in small time scales, correcting accumulated drifts in large time scales (also known as ‘loop closure’), extracting and tracking features from the observed images (e.g. [17, 20]), reducing computational costs of inference (graph-based SLAM [9]) and more.
Visual relocalization is a fundamental task in computer vision. With various applications in robotics, autonomous driving, and virtual/augmented reality, visual relocalization has been studied for decades and a considerable amount of outstanding geometry-based systems have been developed \cite{Taira_2018_CVPR, Toft_2018_ECCV, liu2017efficient, sattler2017efficient, sattler2016large}. Recently, with the success of deep learning techniques in numerous computer vision tasks, global poses can be predicted by exploiting Convolutional Neural Networks (CNNs) \cite{brahmbhatt2018mapnet, kendall2016modelling, kendall2017geometric, melekhov2017hourglass} and Recurrent Neural Networks (RNNs) \cite{ walch2017pose-lstm, clark2017vidloc} in an end-to-end fashion. Most of these methods recover camera poses from single images. It is not easy to estimate poses based on single images because the information is insufficient. Other issues such as noise, texture-less regions, repetitive textures, over-exposure may further aggravate the situation.  As videos provide spatio-temporal consistency over consecutive frames, they are more informative so as to overcome the limitations of single images.
%  While on most platforms including mobile-phones, robots, drones, self-driving cars, image sequences can be readily obtained and frequently utilized in tasks such as visual odometry (VO) and SLAM (Simultaneous Localization And Mapping). 

%Conventionally, the camera pose of a query image can be estimated approximately using the most similar image provided in the database. As images in the database are often sparse, the estimated poses of query images which are far from those in database would be inaccurate. The problem can be partially solved by recovering a global 3D model of the scene, which can be obtained from SfM (Structure from Motion). Given the global model, 2D-3D correspondences between features in the query image and 3D points can be established so that the pose can be calculated by applying RANSAC in combination with a Perspective-n-Point algorithm. Though global information boosts the localization, descriptor matching is time-consuming and ambiguous due to the local similarity \cite{li2012worldwide}. These challenges degrade the performance of the structure-based methods in large-scale environments, such as the urban areas.

\begin{figure}[t]
		%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
		\includegraphics[width=1.\linewidth]{images/overview6}
	\caption{Overview of our framework. Sequential images are first encoded as high-level features which are then fed into the convolutional LSTM \cite{xingjian2015convolutional} for VO estimation. These features are augmented individually by searching co-visibility from hidden states in recurrent units before they are fed into the estimator for global pose regression. Predicted poses are optimized within a pose graph in which the predicted global poses and relative poses represent the nodes and edges, respectively.} 
	\label{fig:framework}
\end{figure}

In order to make full use of the spatial-temporal consistency, we delve into the nature of videos in terms of observations and motions. First, in contrast to single images, videos can build local maps including contents from sequential frames recorded in different viewpoints \cite{schonberger2016colmap}. Thus, they provide wider field of view and more stable features. Ambiguities of single images can be alleviated by using local maps. Additionally, owing to the continuity of camera motions in a video, the relative poses of consecutive frames can be calculated with promising accuracy \cite{mur2017orb-slam2, engel2018dso}. Therefore, these relative poses can be exploited as additional constraints to mitigate the uncertainty that global poses undergo. 

Inspired by classic graph-based SLAM systems \cite{mur2017orb-slam2}, we propose to learn camera relocalization from videos by incorporating a deep VO component. The VO sub-network accepts sequential images as input and predicts relative poses between consecutive frames. The hidden states that record the information of the sequence are taken as local maps. Specifically, our model learns camera relocalization by employing a two-step strategy. First, rather than raw features, the \textit{content}-augmentation step calculates global poses from the features which are enhanced according to the co-visibility in local maps. Moreover, the \textit{motion-}based refinement takes VO results as constraints to enforce the motion consistency of predicted global camera poses within a pose graph during both the training and testing processes. 

% These relative poses are .The global pose regression, however, undergoes uncertainty but is drift-free. Consequently, the VO results and global poses can be tightly coupled and optimized within a pose graph frequently used in current SLAM systems \cite{mur2017orb-slam2} during both the training and testing process. In this manner, camera re-localization and visual odometry can benefit from each other, leading to a win-win situation. As all the results are provided by the model itself, no extra information is required as previous methods \cite{brahmbhatt2018mapnet}. 
%, although VO estimation suffers error accumulation over long sequence.

% the VO results can be utilized as the marginalization to enforce the global consistency of the predicted camera localization, while the global poses can be used as landmark constraint to reduce the error accumulation of visual odometry. During training process, the global and relative poses are optimized mutually. For inference, the VO results are used as constraints to optimize global poses within a pose graph. In this manner, camera re-localization and visual odometry can benefit from each other, leading to a win-win situation.

%which enhances the performance of the whole system. We take inspiration from current classic SLAM systems \cite{mur2017orb-slam2, engel2018dso} by incorporating a pose-graph optimization to enforce the pose consistency over the predicted camera poses. 

The overview of our architecture is shown in Fig.~\ref{fig:framework}. The encoder extracts features from images. The VO sub-network takes sequential features as input and calculates relative poses using convolutional LSTMs (Long Short-Term Memory) \cite{xingjian2015convolutional}. Next, raw features of each view are augmented by searching co-visibility from hidden states using a soft attention. The augmented contents are then fed into the pose predictor to regress camera poses for each view respectively. Finally, with vertexes indicating global poses and  edges representing relative poses, a pose graph is established to enforce the consistency of predicted results. Our contributions can be summarized as follows:

% In this paper, we propose to couple the localization and view generation in a unified model by sharing the same map. The two sub-models are trained jointly with sharing features, so that each sub-model can be inferred individually. Partially inspired by the cycle loss used to maintain the consistency between two sub-tasks \cite{zhu2017cycle-gan, godard2017mono-depth}, we incorporate a cycle loss function over the predicted camera pose and recovered image. Our contributions can be summarized as follows:

\begin{itemize}
	%\item We propose to take advantages of spatio-temporal consistency of videos for camera relocalization by incorporating a VO component.
	%\item Global poses are estimated from the augmented content based on the co-visibility in local maps.
	%\item Global poses are further optimized with VO results as constraints within a pose graph to guarantee the consistency.
	\item We propose to taken advantages of the local information in videos to support global camera poses estimation by incorporating a VO component.
	\item Instead of raw features, our model estimates global poses from contents augmented  based on co-visibility in local maps.
	\item To guarantee the consistency, we adopt the VO results as additional constraints to optimize global poses within a pose graph during training and testing processes.
\end{itemize}

Our approach outperforms current state-of-the-art methods in both the indoor 7-Scenes and outdoor Oxford RobotCar benchmark datasets, especially in challenging scenarios. The rest of this paper is organized as follows. In Sec.~\ref{related_work}, related works on relocalization and visual odometry are introduced. In Sec.~\ref{method}, our framework is described in detail. The performance of our approach is compared with previous methods in Sec.~\ref{experiment}. We conclude the paper in Sec.~\ref{conclusion}.  

%cThe VO estimation between consecutive frames is relatively accurate owing to \textit{small baseline}, but suffers from error accumulation. The single-view global pose prediction is prone inaccurate due to local uncertainty, but gets rid of error accumulation.

%Focusing on alleviating the limitations of classic algorithms, these methods leverage CNNs for place recognition \cite{Balntas_2018_ECCV, Taira_2018_CVPR}, 2D-3D matching \cite{brachmann2017dsac, Brachmann_2018_CVPR, brachmann2016uncertainty}, semantics embedding \cite{Sattler_2018_CVPR, Schonberger_2018_CVPR, Wang_2018_CVPR, Toft_2018_ECCV} or estimating poses directly in an end-to-end fashion \cite{brahmbhatt2018mapnet, kendall2016modelling, kendall2017geometric, walch2017pose-lstm, melekhov2017hourglass, kendall2015posenet}. Due to the finite information of a single image and the lack of global structures, these methods frequently suffer from high ambiguity, especially in challenging scenes, where textures are insufficient or highly repeated.


% Instead of modeling the temporal consistency simply using a regular LSTM (Long Short-Term Memory), which is incapable of tracking long dependencies \cite{sukhbaatar2015memory}, we incorporate a memory module to enhance the ability for preserving global information.  

%Visual localization is a fundamental task in computer vision with various applications for mobile robotics, autonomous driving and virtual/augmented reality. Generally, image-based localization focus on regressing the corresponding 6-DoF camera poses in the world coordinate by given the input images and a map. The map is a implicit/explicit representation of the 3D environments, assisting to track in specific tasks including SLAM (Simultaneous Localization And Mapping) systems \cite{mur2017orb-slam2, engel2018dso}. The elements of maps are generally defined according to specific applications. Points are frequently utilized in general SLAM systems \cite{mur2017orb-slam2, engel2018dso}, as well as structural features including lines \cite{pumarola2017pl-slam} and planes \cite{yang2016pop-slam}. Besides, objects-level \cite{mccormac2018fusion++} and pixel-wise semantics \cite{lianos2018vso, schonberger2018svl} are introduced to handle the challenges such as changing illumination and texture-less regions.

% Inspired by the outstanding performance of convolutional neural networks (CNNs) in many computer vision tasks \cite{he2016resnet}, a variety of excellent algorithms have been proposed to tackle the problem using CNNs in an end-to-end fashion \cite{ brahmbhatt2018mapnet, kendall2016modelling, kendall2017geometric, walch2017pose-lstm, melekhov2017hourglass}. Unlike geometry-based works, in which maps are represented explicitly, and thus explainable, maps in these works are organized as part of the pre-trained weights. Despite their promising results, the map they claimed is utilized to bridge the gap between input observations and corresponding global poses. In contrast, we delve into the nature of maps. In essence, a good map abstracting the 3D environments can not only assist localization but generate views according to the inputs. In specific, the poses can be calculated by giving the map and observations, while the observations can also be recovered providing the poses and the same map. The two sub-tasks can be tacked jointly via sharing a single map. With another constraint, the map can be more representative, and thus boosts the performance of each sub-model. 




==> Sections/Introduction.tex <==
\section{Introduction}
\label{introduction}

%The problem of identifying the position of the camera that captured an image of a scene has been studied extensively for decades [34, 33, 4]. With applications in domains such as robotics and autonomous driving, a considerable amount of engineering effort has been dedicated to developing systems for different versions of the problem. One formulation, often referred to as simply ‘localization’, assumes that a map of the 3D scene is provided in advance and the goal is to localize any new image of the scene relative to this map. A second formulation, commonly referred to as ‘Simultaneous Localization and Mapping’ (SLAM), assumes that there is no prespecified map of the scene, and that it should be estimated concurrently with the locations of each observed image. Research on this topic has focused on different aspects and challenges including: estimating the displacement between frames in small time scales, correcting accumulated drifts in large time scales (also known as ‘loop closure’), extracting and tracking features from the observed images (e.g. [17, 20]), reducing computational costs of inference (graph-based SLAM [9]) and more.
Estimating camera poses from captured images, visual relocalization  is a fundamental task in computer vision. With various applications in robotics, autonomous driving, and virtual/augmented reality, visual relocalization has been studied for decades and a considerable amount of outstanding systems have been developed \cite{brahmbhatt2018mapnet, kendall2016modelling, kendall2017geometric, walch2017pose-lstm, melekhov2017hourglass, Sattler_2018_CVPR, Schonberger_2018_CVPR, Wang_2018_CVPR, Toft_2018_ECCV}. Recently, with the success of deep learning techniques in numerous computer vision tasks, Convolutional Neural Networks (CNNs) and Recurrent Neural Networks (RNNs) are exploited to localize cameras \cite{ brahmbhatt2018mapnet, kendall2016modelling, kendall2017geometric, walch2017pose-lstm, melekhov2017hourglass, clark2017vidloc} in an  end-to-end fashion. Most of these methods recover the camera pose from a single image.  A single image, however, could be knowledge-insufficient due to noise, image-blur, over-exposure, \etal, leading to poor pose prediction. While on most platforms including mobile-phones, robots, drones, self-driving cars, image sequences can be readily obtained and frequently utilized in tasks such as visual odometry (VO) and SLAM (Simultaneous Localization And Mapping). As videos provide spatio-temporal consistency over consecutive frames, they have the potential to enhance the performance of camera relocalization.

%Conventionally, the camera pose of a query image can be estimated approximately using the most similar image provided in the database. As images in the database are often sparse, the estimated poses of query images which are far from those in database would be inaccurate. The problem can be partially solved by recovering a global 3D model of the scene, which can be obtained from SfM (Structure from Motion). Given the global model, 2D-3D correspondences between features in the query image and 3D points can be established so that the pose can be calculated by applying RANSAC in combination with a Perspective-n-Point algorithm. Though global information boosts the localization, descriptor matching is time-consuming and ambiguous due to the local similarity \cite{li2012worldwide}. These challenges degrade the performance of the structure-based methods in large-scale environments, such as the urban areas.

\begin{figure}[t]
	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
		\includegraphics[width=1.\linewidth]{images/overview4}
	\end{center}
	\label{fig:framework}
	\caption{Overview of our framework. The model jointly learns camera relocalization and visual odometry from videos in a unified network. Sequential images are first encoded as high-level features which are then fed into the CNN and ConvLSTM \cite{xingjian2015convolutional} for initial global pose regression and visual odometry (VO) estimation, respectively. The \textit{content}-based refinement ameliorates the initial pose of each view by extracting co-visibility from hidden states in the VO stream with the guidance of corresponding pose features. Additionally, both the refined poses and VO results are further optimized within a pose graph, where the visual odometry estimation represents the edges connecting consecutive refined poses.} 
\end{figure}

 

To make fully use of the spatial-temporal consistency, we analyze the problem from two aspects. First, in contrast to a single image, the video provides more observations from a serious of highly overlapped frames. The co-visible contents over these views are expected to mitigate the challenges including noise, occlusions, repetitive textures in a single image. Additionally, owing to the continuity of camera motions, the relative poses of consecutive frames can be calculated with high accuracy \cite{wang2017deepvo, xue2018fea}, although VO estimation suffers error accumulation over long sequence. The global pose regression, however, undergoes uncertainty but is drift-free. Consequently, the VO results and global poses can be tightly coupled and optimized within a pose graph frequently used in current SLAM systems \cite{mur2017orb-slam2} during both the training and testing process. In this manner, camera re-localization and visual odometry can benefit from each other, leading to a win-win situation. As all the results are provided by the model itself, no extra information is required as previous methods \cite{brahmbhatt2018mapnet}. 

% the VO results can be utilized as the marginalization to enforce the global consistency of the predicted camera localization, while the global poses can be used as landmark constraint to reduce the error accumulation of visual odometry. During training process, the global and relative poses are optimized mutually. For inference, the VO results are used as constraints to optimize global poses within a pose graph. In this manner, camera re-localization and visual odometry can benefit from each other, leading to a win-win situation.

%which enhances the performance of the whole system. We take inspiration from current classic SLAM systems \cite{mur2017orb-slam2, engel2018dso} by incorporating a pose-graph optimization to enforce the pose consistency over the predicted camera poses. 

The overview of our architecture is shown in Fig.~\ref{fig:framework}. The encoder extracts high-level features from images. The relocalization sub-network gives initial pose prediction from these features. Meanwhile, the VO sub-network takes sequential features as input and produces relative poses using convolutional LSTMs (Long Short-Term Memory) \cite{xingjian2015convolutional}. Next, the feature of each view is augmented by searching co-visibility from hidden states using a soft attention with itself as guidance. The augmented contents are fed into pose predictor to calculate refined poses for each view respectively. Finally, with vertexes indicating global poses and relative poses representing edges, a pose graph is established to enforce the global consistency of predicted results. Our contributions can be summarized as follows:

% In this paper, we propose to couple the localization and view generation in a unified model by sharing the same map. The two sub-models are trained jointly with sharing features, so that each sub-model can be inferred individually. Partially inspired by the cycle loss used to maintain the consistency between two sub-tasks \cite{zhu2017cycle-gan, godard2017mono-depth}, we incorporate a cycle loss function over the predicted camera pose and recovered image. Our contributions can be summarized as follows:

\begin{itemize}
	\item We propose to learn the camera relocalization and visual odometry estimation jointly from video clips with a unified model in an end-to-end fashion.
	\item The global pose regression is improved by augmenting the content of a single image based on the co-visibility in feature space. 
	\item The VO results and global poses are exploited tightly coupled within a pose graph and optimized during both the training and testing processes.  
\end{itemize}

Our approach outperforms current state-of-the-art methods in both the indoor 7-Scenes and outdoor Oxford RobotCar benchmark datasets. The rest of this paper is organized as follows. In Sec.\ref{related_work}, related works on relocalization and visual odometry are introduced. In Sec.\ref{method}, our architecture is described in detail. The performance of our approach is compared with previous methods in Sec.\ref{experiment}. We conclude the paper in Sec.\ref{conclusion}.  

%cThe VO estimation between consecutive frames is relatively accurate owing to \textit{small baseline}, but suffers from error accumulation. The single-view global pose prediction is prone inaccurate due to local uncertainty, but gets rid of error accumulation.

%Focusing on alleviating the limitations of classic algorithms, these methods leverage CNNs for place recognition \cite{Balntas_2018_ECCV, Taira_2018_CVPR}, 2D-3D matching \cite{brachmann2017dsac, Brachmann_2018_CVPR, brachmann2016uncertainty}, semantics embedding \cite{Sattler_2018_CVPR, Schonberger_2018_CVPR, Wang_2018_CVPR, Toft_2018_ECCV} or estimating poses directly in an end-to-end fashion \cite{brahmbhatt2018mapnet, kendall2016modelling, kendall2017geometric, walch2017pose-lstm, melekhov2017hourglass, kendall2015posenet}. Due to the finite information of a single image and the lack of global structures, these methods frequently suffer from high ambiguity, especially in challenging scenes, where textures are insufficient or highly repeated.


% Instead of modeling the temporal consistency simply using a regular LSTM (Long Short-Term Memory), which is incapable of tracking long dependencies \cite{sukhbaatar2015memory}, we incorporate a memory module to enhance the ability for preserving global information.  

%Visual localization is a fundamental task in computer vision with various applications for mobile robotics, autonomous driving and virtual/augmented reality. Generally, image-based localization focus on regressing the corresponding 6-DoF camera poses in the world coordinate by given the input images and a map. The map is a implicit/explicit representation of the 3D environments, assisting to track in specific tasks including SLAM (Simultaneous Localization And Mapping) systems \cite{mur2017orb-slam2, engel2018dso}. The elements of maps are generally defined according to specific applications. Points are frequently utilized in general SLAM systems \cite{mur2017orb-slam2, engel2018dso}, as well as structural features including lines \cite{pumarola2017pl-slam} and planes \cite{yang2016pop-slam}. Besides, objects-level \cite{mccormac2018fusion++} and pixel-wise semantics \cite{lianos2018vso, schonberger2018svl} are introduced to handle the challenges such as changing illumination and texture-less regions.

% Inspired by the outstanding performance of convolutional neural networks (CNNs) in many computer vision tasks \cite{he2016resnet}, a variety of excellent algorithms have been proposed to tackle the problem using CNNs in an end-to-end fashion \cite{ brahmbhatt2018mapnet, kendall2016modelling, kendall2017geometric, walch2017pose-lstm, melekhov2017hourglass}. Unlike geometry-based works, in which maps are represented explicitly, and thus explainable, maps in these works are organized as part of the pre-trained weights. Despite their promising results, the map they claimed is utilized to bridge the gap between input observations and corresponding global poses. In contrast, we delve into the nature of maps. In essence, a good map abstracting the 3D environments can not only assist localization but generate views according to the inputs. In specific, the poses can be calculated by giving the map and observations, while the observations can also be recovered providing the poses and the same map. The two sub-tasks can be tacked jointly via sharing a single map. With another constraint, the map can be more representative, and thus boosts the performance of each sub-model. 




==> fig_tables/PlotFigOfScenses.tex <==
\def\subfig_width{0.25\textwidth}
\def\PlotFigOfScenses#1#2#3#4{
	\begin{subfigure}{#4}
		%\includegraphics[width=1\textwidth]{images/results_7scenes/pose/dso/#1-dso-seq-#2.pdf}
		\includegraphics[width=0.95\textwidth]{images/dataset/7scenes/#1.png}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{#4}
		\includegraphics[width=1\textwidth]{images/results_7scenes/pose/posenet/posenet_#1_#3_pose.pdf}
		\centerline{\includegraphics[width=1\textwidth]{images/results_7scenes/rot/posenet/posenet_#1_#3_rot.pdf}}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{#4}
		\includegraphics[width=1\textwidth]{images/results_7scenes/pose/mapnet/mapnet_#1_#3_pose.pdf}
		\centerline{\includegraphics[width=1\textwidth]{images/results_7scenes/rot/mapnet/mapnet_#1_#3_rot.pdf}}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{#4}
		\includegraphics[width=1\textwidth]{images/results_7scenes/pose/mapnet++/mapnet++_#1_#3_pose.pdf}
		\centerline{\includegraphics[width=1\textwidth]{images/results_7scenes/rot/mapnet++/mapnet++_#1_#3_rot.pdf}}
	\end{subfigure}
	%-------------------rot---------------------
	%\begin{subfigure}[h]{#4}
	%	\includegraphics[width=1\textwidth]{images/results_7scenes/rot/dso/#1-dso-seq-#2.pdf}
	%\end{subfigure}%
	%\hfill
	%\begin{subfigure}[h]{#4}
	%	\includegraphics[width=1\textwidth]{images/results_7scenes/rot/posenet/posenet_#1_#3_rot.pdf}
	%\end{subfigure}%
	%\hfill
	%\begin{subfigure}[h]{#4}
	%	\includegraphics[width=1\textwidth]{images/results_7scenes/rot/mapnet/mapnet_#1_#3_rot.pdf}
	%\end{subfigure}%
	%\hfill
	%\begin{subfigure}[h]{#4}
	%	\includegraphics[width=1\textwidth]{images/results_7scenes/rot/mapnet++/mapnet++_#1_#3_rot.pdf}
	%\end{subfigure}
	%--------------------------------------
	}


==> fig_tables/fig_robotcar_full.tex <==
\begin{figure*}[t]
\def\subfig_width{0.25}
\centering
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/results/Stereo-2014-12-09-13-21-02.pdf}
	\centerline{Stereo VO (222.0m, $13.7^\circ$)}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/results/posenet-2014-12-09-13-21-02.pdf}
	\centerline{PoseNet (125.6m, $27.1^\circ$)}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/results/mapnet-2014-12-09-13-21-02.pdf}
	\centerline{MapNet (41.4m, $12.5^\circ$)}
	%\label{fig:trajectory_kitti_00_07}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/results/mapnet-2014-12-09-13-21-02.pdf}
	\centerline{Ours (40.20m, $12.85^\circ$)}
	%\label{fig:trajectory_kitti_00_10_10}
\end{subfigure}
	\caption{Results of Stereo VO, PoseNet \cite{kendall2015posenet}, MapNet \cite{brahmbhatt2018mapnet} and our model on the FULL route (9562m) of the Oxford RobotCar dataset \cite{robotcar2017} (red line indicates predicted poses and block line represents the ground truth poses). Results of Stereo VO are provided by the dataset. Predicted poses of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. The caption of each figure shows the mean translation error (m) and mean rotation error ($\circ$).}
	\label{fig:exp_robotcar_full}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/fig_robotcar_full_extend.tex <==
\begin{figure*}[t]
	
\def\subfig_width{0.25}
\def\seq_name{2014-12-05-11-09-10}
\centering
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/Stereo-\seq_name.pdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-50.pdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-50.pdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-50.pdf}
\end{subfigure}%

% 2 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_trans_cdf.pdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-100.pdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-100.pdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-100.pdf}
\end{subfigure}%

% 3 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_rot_cdf.pdf}
	\centerline{Cumulative errors.}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-150.pdf}
	\centerline{PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}.}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-150.pdf}
	\centerline{MapNet \cite{brahmbhatt2018mapnet}.}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-150.pdf}
	\centerline{Ours.}
\end{subfigure}%

\caption{Results of Stereo VO, PoseNet, MapNet and our model on the FULL3 scenes of the Oxford RobotCar dataset \cite{robotcar2017} The red and black lines indicate predicted and ground truth poses respectively. The star represents the start point. Results of Stereo VO are provided by the dataset. The poses of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. To better visualize the trajectories, we select points with translation errors within 50m (top), 100m (middle) and 150m (bottom). Cumulative translation (middle left) and rotation (bottom left) errors are also illustrated.}
	% The caption of each figure shows the mean translation error (m) and mean rotation error ($\circ$)
	\label{fig:exp_robotcar_110910}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/fig_robotcar_full_extend_084510.tex <==
\begin{figure*}[t]
	
\def\subfig_width{0.25}
\def\seq_name{2015-02-03-08-45-10}
\centering
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/Stereo-\seq_name}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-50}
\end{subfigure}%

% 2 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_trans_cdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-100}
\end{subfigure}%

% 3 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_rot_cdf}
	\centerline{Cumulative errors}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-150}
	\centerline{PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-150}
	\centerline{MapNet \cite{brahmbhatt2018mapnet}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-150}
	\centerline{Ours}
\end{subfigure}%

\caption{Results of Stereo VO, PoseNet, MapNet and our model on the FULL5 scenes of the Oxford RobotCar dataset \cite{robotcar2017} The red and black lines indicate predicted and ground truth poses respectively. The star represents the start point. Results of Stereo VO are provided by the dataset. The poses of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. To better visualize the trajectories, we select points with translation errors within 50m (top), 100m (middle) and 150m (bottom). Cumulative translation (middle left) and rotation (bottom left) errors are also illustrated.}
	% The caption of each figure shows the mean translation error (m) and mean rotation error ($\circ$)
	\label{fig:exp_robotcar_084510}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/fig_robotcar_full_extend_091832.tex <==
\begin{figure*}[t]
	
\def\subfig_width{0.25}
\def\seq_name{2014-11-25-09-18-32}
\centering
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/Stereo-\seq_name}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-50}
\end{subfigure}%

% 2 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_trans_cdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-100}
\end{subfigure}%

% 3 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_rot_cdf}
	\centerline{Cumulative errors}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-150}
	\centerline{PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-150}
	\centerline{MapNet \cite{brahmbhatt2018mapnet}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-150}
	\centerline{Ours}
\end{subfigure}%

\caption{Results of Stereo VO, PoseNet, MapNet and our model on the FULL4 scenes of the Oxford RobotCar dataset \cite{robotcar2017} The red and black lines indicate predicted and ground truth poses respectively. The star represents the start point. Results of Stereo VO are provided by the dataset. The poses of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. To better visualize the trajectories, we select points with translation errors within 50m (top), 100m (middle) and 150m (bottom). Cumulative translation (middle left) and rotation (bottom left) errors are also illustrated.}
	% The caption of each figure shows the mean translation error (m) and mean rotation error ($\circ$)
	\label{fig:exp_robotcar_091832}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/fig_robotcar_full_extend_110910.tex <==
\begin{figure*}[t]
	
\def\subfig_width{0.25}
\def\seq_name{2014-12-05-11-09-10}
\def\img_format{}
\centering
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/Stereo-\seq_name\img_format}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-50\img_format}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-50\img_format}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-50\img_format}
\end{subfigure}%

% 2 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_trans_cdf.pdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-100\img_format}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-100\img_format}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-100\img_format}
\end{subfigure}%

% 3 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_rot_cdf.pdf}
	\centerline{Cumulative errors.}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-150\img_format}
	\centerline{PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-150\img_format}
	\centerline{MapNet \cite{brahmbhatt2018mapnet}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-150\img_format}
	\centerline{Ours}
\end{subfigure}%

\caption{Results of Stereo VO, PoseNet, MapNet and our model on the FULL3 scenes of the Oxford RobotCar dataset \cite{robotcar2017} The red and black lines indicate predicted and ground truth poses respectively. The star represents the start point. Results of Stereo VO are provided by the dataset. The poses of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. To better visualize the trajectories, we select points with translation errors within 50m (top), 100m (middle) and 150m (bottom). Cumulative translation (middle left) and rotation (bottom left) errors are also illustrated.}
	% The caption of each figure shows the mean translation error (m) and mean rotation error ($\circ$)
	\label{fig:exp_robotcar_110910}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/fig_robotcar_full_extend_123219.tex <==
\begin{figure*}[t]
	
\def\subfig_width{0.25}
\def\seq_name{2015-02-24-12-32-19}
\centering
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/Stereo-\seq_name}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-50}
\end{subfigure}%

% 2 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_trans_cdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-100}
\end{subfigure}%

% 3 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_rot_cdf}
	\centerline{Cumulative errors}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-150}
	\centerline{PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-150}
	\centerline{MapNet \cite{brahmbhatt2018mapnet}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-150}
	\centerline{Ours}
\end{subfigure}%

\caption{Results of Stereo VO, PoseNet, MapNet and our model on the FULL6 scenes of the Oxford RobotCar dataset \cite{robotcar2017} The red and black lines indicate predicted and ground truth poses respectively. The star represents the start point. Results of Stereo VO are provided by the dataset. The poses of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. To better visualize the trajectories, we select points with translation errors within 50m (top), 100m (middle) and 150m (bottom). Cumulative translation (middle left) and rotation (bottom left) errors are also illustrated.}
	% The caption of each figure shows the mean translation error (m) and mean rotation error ($\circ$)
	\label{fig:exp_robotcar_123219}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/fig_robotcar_full_extend_181050.tex <==
\begin{figure*}[t]
	
\def\subfig_width{0.25}
\def\seq_name{2014-12-10-18-10-50}
\centering
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/Stereo-\seq_name}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-50}
\end{subfigure}%

% 2 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_trans_cdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-100}
\end{subfigure}%

% 3 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_rot_cdf}
	\centerline{Cumulative errors}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-150}
	\centerline{PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-150}
	\centerline{MapNet \cite{brahmbhatt2018mapnet}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-150}
	\centerline{Ours}
\end{subfigure}%

\caption{Results of Stereo VO, PoseNet, MapNet and our model on the FULL7 scenes of the Oxford RobotCar dataset \cite{robotcar2017} The red and black lines indicate predicted and ground truth poses respectively. The star represents the start point. Results of Stereo VO are provided by the dataset. The poses of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. To better visualize the trajectories, we select points with translation errors within 50m (top), 100m (middle) and 150m (bottom). Cumulative translation (middle left) and rotation (bottom left) errors are also illustrated.}
	% The caption of each figure shows the mean translation error (m) and mean rotation error ($\circ$)
	\label{fig:exp_robotcar_181050}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/fig_robotcar_full_extend_181843.tex <==
\begin{figure*}[t]
	
\def\subfig_width{0.25}
\def\seq_name{2014-12-17-18-18-43}
\centering
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/Stereo-\seq_name}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-50}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-50}
\end{subfigure}%

% 2 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_trans_cdf}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-100}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-100}
\end{subfigure}%

% 3 row
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/cdf/\seq_name_rot_cdf}
	\centerline{Cumulative errors}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/posenet-\seq_name-clip_t-150}
	\centerline{PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/mapnet-\seq_name-clip_t-150}
	\centerline{MapNet \cite{brahmbhatt2018mapnet}}
\end{subfigure}%
\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=1\textwidth]{images/pvnet-select_crop/extend/pose/pvnet_e58_v0-\seq_name-clip_t-150}
	\centerline{Ours}
\end{subfigure}%

\caption{Results of Stereo VO, PoseNet, MapNet and our model on the FULL8 scenes of the Oxford RobotCar dataset \cite{robotcar2017} The red and black lines indicate predicted and ground truth poses respectively. The star represents the start point. Results of Stereo VO are provided by the dataset. The poses of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. To better visualize the trajectories, we select points with translation errors within 50m (top), 100m (middle) and 150m (bottom). Cumulative translation (middle left) and rotation (bottom left) errors are also illustrated.}
	% The caption of each figure shows the mean translation error (m) and mean rotation error ($\circ$)
	\label{fig:exp_robotcar_181843}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/fig_vis_samples.tex <==
\begin{figure*}[t]
	\def\subfig_width{0.195}
	%\setlength{\abovecaptionskip}{-1cm}
	%\setlength{\belowcaptionskip}{-1cm}
\centering
% for posenet
\begin{subfigure}{1.0\textwidth}
	\centering
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/posenet/frame_411.png}
	%\subcaption{December, overcast}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/posenet/frame_1400.png}
	%\subcaption{November, rain}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/posenet/frame_1608.png}
	%\subcaption{February, snow}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/posenet/frame_2094.png}
	%\subcaption{December, night}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/posenet/frame_2160.png}
%	\subcaption{Febreuary, roadworks}
\subcaption{Attention maps of example images for PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}.}
\end{subfigure}%
\vspace{0.2cm}

% for mapnet
\begin{subfigure}{1.0\textwidth}
	\centering
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/mapnet/frame_411.png}
	%\subcaption{December, overcast}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/mapnet/frame_1400.png}
	%\subcaption{November, rain}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/mapnet/frame_1608.png}
	%\subcaption{February, snow}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/mapnet/frame_2094.png}
	%\subcaption{December, night}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/mapnet/frame_2160.png}
	\subcaption{Attention maps of example images for MapNet \cite{brahmbhatt2018mapnet}.}
	%	\subcaption{Febreuary, roadworks}
\end{subfigure}%
\vspace{0.2cm}
% for pvnet
\begin{subfigure}{1.\textwidth}
	\centering
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/pvnet/frame_411.png}
	%\subcaption{December, overcast}
%\end{subfigure}%
%\begin{subfigure}{1.\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/pvnet/frame_1400.png}
	%\subcaption{November, rain}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/pvnet/frame_1608.png}
	%\subcaption{February, snow}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/pvnet/frame_2094.png}
	%\subcaption{December, night}
%\end{subfigure}%
%\begin{subfigure}{\subfig_width\textwidth}
	\includegraphics[width=\subfig_width\textwidth]{images/samples/vis/pvnet/frame_2160.png}
	\subcaption{Attention maps of example images for our model.}
	%	\subcaption{Febreuary, roadworks}
\end{subfigure}%

\caption{Attention maps of example images for (a) PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}, (b) MapNet \cite{brahmbhatt2018mapnet} and (c) our model on Oxford RobotCar dataset \cite{robotcar2017}. Compared with PoseNet and MapNet, our model focuses more on static objects and regions with geometric meanings (Fig.~\ref{fig:vis_b, fig:vis_e}). Both local and global are concentrated in our method to mitigate local similar appearances. Moreover, our salient maps are more consistent over time.}
\label{fig:vis_samples}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}


==> fig_tables/table_7scenes.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
\setlength{\tabcolsep}{4.pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table*}[t]
	%\scriptsize
	\footnotesize
	%\small
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{lcccccccc}
				\hline
				\hline
				& \multicolumn{8}{c}{Sequence} \\
				% \cline{2-15} 
				%Method & \multicolumn{2}{c}{03} & \multicolumn{2}{c}{04} & \multicolumn{2}{c}{05} & \multicolumn{2}{c}{06} & \multicolumn{2}{c}{07} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{Avg}\\ 
				Method & Chess & Fire & Heads & Office & Pumpkin & Kitchen & Stairs & Avg \\
				%Method & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} &  \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} \\
				%& $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$   \\
				\hline
				% DeepVO &  \multicolumn{2}{c} {$- \quad -$} &  \multicolumn{2}{c}{$8.49 \quad 6.89$} &  \multicolumn{2}{c}{$7.19 \quad 6.97$} &  \multicolumn{2}{c}{$2.62 \quad 3.61$} &  \multicolumn{2}{c}{$5.42 \quad 5.82$} &  \multicolumn{2}{c}{$3.91 \quad 4.60$} &  \multicolumn{2}{c}{$8.11 \quad 8.83$} \\
				
				%PoseNet15 \cite{kendall2015posenet} & 0.32m, $4.06^\circ$ & 0.47m, $7.33^\circ$ & 0.29m, $6.00^\circ$ & 0.48m, $3.84^\circ$ & 0.47m, $4.21^\circ$ & 0.59m, $4.32^\circ$ & 0.47m, $6.93^\circ$ & 0.44m, $10.4^\circ$ \\
				PoseNet15 \cite{kendall2015posenet} & 0.32
				m, $8.12^\circ$ & 0.47m, $14.4^\circ$ & 0.29m, $12.0^\circ$ & 0.48m, $7.68^\circ$ & 0.47m, $8.42^\circ$ & 0.59m, $8.64^\circ$ & 0.47m, $13.8^\circ$ & 0.44m, $10.4^\circ$ \\
				PoseNet16 \cite{kendall2016modelling} & 0.37
				m, $7.24^\circ$ & 0.43m, $13.7^\circ$ & 0.31m, $12.0^\circ$ & 0.48m, $8.04^\circ$ & 0.61m, $7.08^\circ$ & 0.58m, $7.54^\circ$ & 0.48m, $13.1^\circ$ & 0.47m, $9.81^\circ$ \\
				PoseNet17 \cite{kendall2017geometric} & 0.13m, $4.48^\circ$ & 0.27m, $11.30^\circ$ & 0.17m, $13.00^\circ$ & 0.19m, $5.55^\circ$ & 0.26m, $4.75^\circ$ & 0.23m, $5.35^\circ$ & 0.35m, $12.40^\circ$ & 0.23m, $8.12^\circ$ \\
				Hourglass \cite{melekhov2017hourglass} & 0.15m, $6.17^\circ$ & 0.27m, $10.84^\circ$ & 0.19m, $11.63^\circ$ & 0.21m, $8.48^\circ$ & 0.25m, $7.01^\circ$ & 0.27m, $10.15^\circ$ & 0.29m, $12.46^\circ$ & 0.23m, $9.53^\circ$ \\
				LSTM-Pose \cite{walch2017pose-lstm} & 0.24m, $5.77^\circ$ & 0.34m, $11.9^\circ$ & 0.21m, $13.7^\circ$ & 0.30m, $8.08^\circ$ & 0.33m, $7.00^\circ$ & 0.37m, $8.83^\circ$ & 0.40m, $13.7^\circ$ & 0.31m, $9.85^\circ$ \\
				VidLoc \cite{clark2017vidloc} & 0.18m, NA & 0.26m, NA & 0.14m, NA & 0.26m, NA & 0.36m, NA & 0.31m, NA & 0.26m, NA & 0.25m, NA \\
				DSO \cite{engel2018dso} & 0.17m, $8.13^\circ$ & 0.19m, $65.0^\circ$ & 0.61m, $68.2^\circ$ & 1.51m, $16.8^\circ$ & 0.61m, $15.8^\circ$ & 0.23m, $10.9^\circ$ & 0.26m, $21.3^\circ$ & 0.26m, $29.4^\circ$ \\
				%ReLocNet \cite{Balntas_2018_ECCV} & 0.12m, $4.14^\circ$ & 0.26m, $10.04^\circ$ & 0.14m, $10.05^\circ$ & 0.18m, $5.32^\circ$ & 0.26m, $4.17^\circ$ & 0.23m, $5.08^\circ$ & 0.28m, $7.53^\circ$ & 1.00m, $1.00^\circ$ \\
				%MapNet \cite{brahmbhatt2018mapnet} & 0.08m, $3.25^\circ$ & 0.27m, $11.69^\circ$ & 0.18m, $13.25^\circ$ & 0.17m, $5.15^\circ$ & 0.22m, $4.02^\circ$ & 0.23m, $4.93^\circ$ & 0.30m, $12.08^\circ$ & 0.21m, $7.77^\circ$ \\
				%MapNet+ \cite{brahmbhatt2018mapnet} & 0.10m, $3.17^\circ$ & 0.20m, $9.04^\circ$ & 0.13m, $11.13^\circ$ & 0.18m, $5.38^\circ$ & 0.19m, $3.92^\circ$ & 0.20m, $5.01^\circ$ & 0.30m, $13.37^\circ$ & 0.19m, $7.29^\circ$ \\
				%MapNet+PGO \cite{brahmbhatt2018mapnet} & 0.09m, $3.24^\circ$ & 0.20m, $9.29^\circ$ & 0.12m, $8.45^\circ$ & 0.19m, $5.42^\circ$ & 0.19m, $3.96^\circ$ & 0.20m, $4.94^\circ$ & 0.27m, $10.57^\circ$ & 0.18m, $6.55^\circ$ \\
				Ours & 0.08m, $3.25^\circ$ & 0.27m, $11.69^\circ$ & 0.17m, $12.70^\circ$ & 0.17m, $5.15^\circ$ & 0.20m, $3.66^\circ$ & 0.23m, $4.93^\circ$ & 0.27m, $10.21^\circ$ & 0.21m, $7.77^\circ$ \\
				\hline
				\hline
			\end{tabular}
		\end{center}
	
	\caption{Result of previous methods and our model on the 7-Scenes dataset \cite{shotton2013scene}. The best results are highlighted.}
	\label{tab:7scenes}
\end{table*}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}

==> fig_tables/table_7scenes_sequence.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
%\setlength{\tabcolsep}{4.pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[t]
	%\scriptsize
	%\footnotesize
	\small
	\centering
	\setlength{\abovecaptionskip}{0pt}%    
	\setlength{\belowcaptionskip}{0pt}%
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{lccc}
				\hline
				\hline
				& \multicolumn{3}{c}{Method} \\
				% \cline{2-15} 
				%Method & \multicolumn{2}{c}{03} & \multicolumn{2}{c}{04} & \multicolumn{2}{c}{05} & \multicolumn{2}{c}{06} & \multicolumn{2}{c}{07} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{Avg}\\ 
				Scene & VidLoc \cite{clark2017vidloc} & MapNet \cite{brahmbhatt2018mapnet}  & \textbf{Ours} \\
				%Method & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} &  \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} \\
				%& $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$   \\
				\hline
				% DeepVO &  \multicolumn{2}{c} {$- \quad -$} &  \multicolumn{2}{c}{$8.49 \quad 6.89$} &  \multicolumn{2}{c}{$7.19 \quad 6.97$} &  \multicolumn{2}{c}{$2.62 \quad 3.61$} &  \multicolumn{2}{c}{$5.42 \quad 5.82$} &  \multicolumn{2}{c}{$3.91 \quad 4.60$} &  \multicolumn{2}{c}{$8.11 \quad 8.83$} \\
				
				Chess & 0.18m, NA &  \textbf{0.08}m, $\mathbf{3.25}^\circ$ & 0.09m, $3.28^\circ$ \\
				Fire & 0.26m, NA & 0.27m, $11.69^\circ$ & \textbf{0.26}m, $\mathbf{10.92}^\circ$ \\
				Heads & \textbf{0.14}m, NA & 0.18m, $13.25^\circ$ & 0.17m, $\mathbf{12.70}^\circ$ \\
				Office & 0.26m, NA & \textbf{0.17}m, $\mathbf{5.15}^\circ$ & 0.18m, $5.45^\circ$ \\
				Pumpkin & 0.36m, NA & 0.22m, $4.02^\circ$ & \textbf{0.20}m, $\mathbf{3.69}^\circ$ \\
				Kitchen & 0.31m, NA & 0.23m, $4.93^\circ$ & \textbf{0.23}m, $\mathbf{4.92}^\circ$ \\
				Stairs & 0.26m, NA & 0.30m, $12.08^\circ$ & \textbf{0.23}m, $\mathbf{11.3}^\circ$\\
				Avg & 0.25m, NA & 0.21m, $7.77^\circ$ & \textbf{0.19}m, $\mathbf{7.47}^\circ$\\
				
				%PoseNet15 \cite{kendall2015posenet} & 0.32m, $4.06^\circ$ & 0.47m, $7.33^\circ$ & 0.29m, $6.00^\circ$ & 0.48m, $3.84^\circ$ & 0.47m, $4.21^\circ$ & 0.59m, $4.32^\circ$ & 0.47m, $6.93^\circ$ & 0.44m, $10.4^\circ$ \\
				%PoseNet16 \cite{kendall2016modelling} & 0.37m, $7.24^\circ$ & 0.43m, $13.7^\circ$ & 0.31m, $12.0^\circ$ & 0.48m, $8.04^\circ$ & 0.61m, $7.08^\circ$ & 0.58m, $7.54^\circ$ & 0.48m, $13.1^\circ$ & 0.47m, $9.81^\circ$ \\
				%PoseNet17 \cite{kendall2017geometric} & 0.13m, $4.48^\circ$ & 0.27m, $11.30^\circ$ & 0.17m, $13.00^\circ$ & 0.19m, $5.55^\circ$ & 0.26m, $4.75^\circ$ & 0.23m, $5.35^\circ$ & 0.35m, $12.40^\circ$ & 0.23m, $8.12^\circ$ \\
				%Hourglass \cite{melekhov2017hourglass} & 0.15m, $6.17^\circ$ & 0.27m, $10.84^\circ$ & 0.19m, $11.63^\circ$ & 0.21m, $8.48^\circ$ & 0.25m, $7.01^\circ$ & 0.27m, $10.15^\circ$ & 0.29m, $12.46^\circ$ & 0.23m, $9.53^\circ$ \\
				%LSTM-Pose \cite{walch2017pose-lstm} & 0.24m, $5.77^\circ$ & 0.34m, $11.9^\circ$ & 0.21m, $13.7^\circ$ & 0.30m, $8.08^\circ$ & 0.33m, $7.00^\circ$ & 0.37m, $8.83^\circ$ & 0.40m, $13.7^\circ$ & 0.31m, $9.85^\circ$ \\
				%VidLoc \cite{clark2017vidloc} & 0.18m, NA & 0.26m, NA & 0.14m, NA & 0.26m, NA & 0.36m, NA & 0.31m, NA & 0.26m, NA & 0.25m, NA \\
				%DSO \cite{engel2018dso} & 0.17m, $8.13^\circ$ & 0.19m, $65.0^\circ$ & 0.61m, $68.2^\circ$ & 1.51m, $16.8^\circ$ & 0.61m, $15.8^\circ$ & 0.23m, $10.9^\circ$ & 0.26m, $21.3^\circ$ & 0.26m, $29.4^\circ$ \\
				%ReLocNet \cite{Balntas_2018_ECCV} & 0.12m, $4.14^\circ$ & 0.26m, $10.04^\circ$ & 0.14m, $10.05^\circ$ & 0.18m, $5.32^\circ$ & 0.26m, $4.17^\circ$ & 0.23m, $5.08^\circ$ & 0.28m, $7.53^\circ$ & 1.00m, $1.00^\circ$ \\
				%MapNet \cite{brahmbhatt2018mapnet} & 0.08m, $3.25^\circ$ & 0.27m, $11.69^\circ$ & 0.18m, $13.25^\circ$ & 0.17m, $5.15^\circ$ & 0.22m, $4.02^\circ$ & 0.23m, $4.93^\circ$ & 0.30m, $12.08^\circ$ & 0.21m, $7.77^\circ$ \\
				%MapNet+ \cite{brahmbhatt2018mapnet} & 0.10m, $3.17^\circ$ & 0.20m, $9.04^\circ$ & 0.13m, $11.13^\circ$ & 0.18m, $5.38^\circ$ & 0.19m, $3.92^\circ$ & 0.20m, $5.01^\circ$ & 0.30m, $13.37^\circ$ & 0.19m, $7.29^\circ$ \\
				%MapNet+PGO \cite{brahmbhatt2018mapnet} & 0.09m, $3.24^\circ$ & 0.20m, $9.29^\circ$ & 0.12m, $8.45^\circ$ & 0.19m, $5.42^\circ$ & 0.19m, $3.96^\circ$ & 0.20m, $4.94^\circ$ & 0.27m, $10.57^\circ$ & 0.18m, $6.55^\circ$ \\
				\hline
				\hline
			\end{tabular}
		\end{center}
	
	\caption{Median translation and rotation errors of VidLoc \cite{clark2017vidloc}, MapNet \cite{brahmbhatt2018mapnet} and  our approach on the 7-Scenes dataset \cite{shotton2013scene}. The best results are highlighted.}
	\label{tab:scenes_sequence}
\end{table}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}

==> fig_tables/table_ablation_7scenes.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
%\setlength{\tabcolsep}{4.pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[t]
	%\scriptsize
	%\footnotesize
	\small
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{lccc}
				\hline
				\hline
				& \multicolumn{3}{c}{Method} \\
				% \cline{2-15} 
				%Method & \multicolumn{2}{c}{03} & \multicolumn{2}{c}{04} & \multicolumn{2}{c}{05} & \multicolumn{2}{c}{06} & \multicolumn{2}{c}{07} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{Avg}\\ 
				Scene & Ours (baseline) & Ours (w/o motion)  & Ours (full) \\
				%Method & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} &  \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} & \multicolumn{2}{c}{$t_{rel} \quad r_{rel}$} \\
				%& $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$ &  $t_{rel}$ & $r_{rel}$   \\
				\hline
				% DeepVO &  \multicolumn{2}{c} {$- \quad -$} &  \multicolumn{2}{c}{$8.49 \quad 6.89$} &  \multicolumn{2}{c}{$7.19 \quad 6.97$} &  \multicolumn{2}{c}{$2.62 \quad 3.61$} &  \multicolumn{2}{c}{$5.42 \quad 5.82$} &  \multicolumn{2}{c}{$3.91 \quad 4.60$} &  \multicolumn{2}{c}{$8.11 \quad 8.83$} \\
				
				Chess & 0.11m, $4.29^\circ$ & 0.47m, $7.33^\circ$ & 0.29m, $6.00^\circ$ \\
				Fire & 0.27m, $12.13^\circ$ & 0.47m, $7.33^\circ$ & 0.29m, $6.00^\circ$ \\
				Heads & 0.19m, $12.15^\circ$ & 0.47m, $7.33^\circ$ & 0.17m, $12.70^\circ$ \\
				Office & 0.19m, $6.35^\circ$ & 0.47m, $7.33^\circ$ & 0.29m, $6.00^\circ$ \\
				Pumpkin & 0.22m, $6.05^\circ$ & 0.47m, $7.33^\circ$ & 0.20m, $3.69^\circ$ \\
				Kitchen & 0.25m, $5.27^\circ$ & 0.47m, $7.33^\circ$ & 0.29m, $6.00^\circ$ \\
				Stairs & 0.30m, $11.29^\circ$ & 0.47m, $7.33^\circ$ & 0.23m, $11.3^\circ$\\
				Avg & 0.22m, $8.07^\circ$ & 0.47m, $7.33^\circ$ & 0.29m, $6.00^\circ$\\
				
				%PoseNet15 \cite{kendall2015posenet} & 0.32m, $4.06^\circ$ & 0.47m, $7.33^\circ$ & 0.29m, $6.00^\circ$ & 0.48m, $3.84^\circ$ & 0.47m, $4.21^\circ$ & 0.59m, $4.32^\circ$ & 0.47m, $6.93^\circ$ & 0.44m, $10.4^\circ$ \\
				%PoseNet16 \cite{kendall2016modelling} & 0.37m, $7.24^\circ$ & 0.43m, $13.7^\circ$ & 0.31m, $12.0^\circ$ & 0.48m, $8.04^\circ$ & 0.61m, $7.08^\circ$ & 0.58m, $7.54^\circ$ & 0.48m, $13.1^\circ$ & 0.47m, $9.81^\circ$ \\
				%PoseNet17 \cite{kendall2017geometric} & 0.13m, $4.48^\circ$ & 0.27m, $11.30^\circ$ & 0.17m, $13.00^\circ$ & 0.19m, $5.55^\circ$ & 0.26m, $4.75^\circ$ & 0.23m, $5.35^\circ$ & 0.35m, $12.40^\circ$ & 0.23m, $8.12^\circ$ \\
				%Hourglass \cite{melekhov2017hourglass} & 0.15m, $6.17^\circ$ & 0.27m, $10.84^\circ$ & 0.19m, $11.63^\circ$ & 0.21m, $8.48^\circ$ & 0.25m, $7.01^\circ$ & 0.27m, $10.15^\circ$ & 0.29m, $12.46^\circ$ & 0.23m, $9.53^\circ$ \\
				%LSTM-Pose \cite{walch2017pose-lstm} & 0.24m, $5.77^\circ$ & 0.34m, $11.9^\circ$ & 0.21m, $13.7^\circ$ & 0.30m, $8.08^\circ$ & 0.33m, $7.00^\circ$ & 0.37m, $8.83^\circ$ & 0.40m, $13.7^\circ$ & 0.31m, $9.85^\circ$ \\
				%VidLoc \cite{clark2017vidloc} & 0.18m, NA & 0.26m, NA & 0.14m, NA & 0.26m, NA & 0.36m, NA & 0.31m, NA & 0.26m, NA & 0.25m, NA \\
				%DSO \cite{engel2018dso} & 0.17m, $8.13^\circ$ & 0.19m, $65.0^\circ$ & 0.61m, $68.2^\circ$ & 1.51m, $16.8^\circ$ & 0.61m, $15.8^\circ$ & 0.23m, $10.9^\circ$ & 0.26m, $21.3^\circ$ & 0.26m, $29.4^\circ$ \\
				%ReLocNet \cite{Balntas_2018_ECCV} & 0.12m, $4.14^\circ$ & 0.26m, $10.04^\circ$ & 0.14m, $10.05^\circ$ & 0.18m, $5.32^\circ$ & 0.26m, $4.17^\circ$ & 0.23m, $5.08^\circ$ & 0.28m, $7.53^\circ$ & 1.00m, $1.00^\circ$ \\
				%MapNet \cite{brahmbhatt2018mapnet} & 0.08m, $3.25^\circ$ & 0.27m, $11.69^\circ$ & 0.18m, $13.25^\circ$ & 0.17m, $5.15^\circ$ & 0.22m, $4.02^\circ$ & 0.23m, $4.93^\circ$ & 0.30m, $12.08^\circ$ & 0.21m, $7.77^\circ$ \\
				%MapNet+ \cite{brahmbhatt2018mapnet} & 0.10m, $3.17^\circ$ & 0.20m, $9.04^\circ$ & 0.13m, $11.13^\circ$ & 0.18m, $5.38^\circ$ & 0.19m, $3.92^\circ$ & 0.20m, $5.01^\circ$ & 0.30m, $13.37^\circ$ & 0.19m, $7.29^\circ$ \\
				%MapNet+PGO \cite{brahmbhatt2018mapnet} & 0.09m, $3.24^\circ$ & 0.20m, $9.29^\circ$ & 0.12m, $8.45^\circ$ & 0.19m, $5.42^\circ$ & 0.19m, $3.96^\circ$ & 0.20m, $4.94^\circ$ & 0.27m, $10.57^\circ$ & 0.18m, $6.55^\circ$ \\
				\hline
				\hline
			\end{tabular}
		\end{center}
	
	\caption{Result of the variations of our model on the 7-Scenes dataset \cite{shotton2013scene}. \textbf{Ours (baseline)} indicates the model without \textit{content} augmentation and \textit{motion}-based refinement. \textbf{Ours (w/o motion)} denotes the model with \textit{content} augmentation but without \textit{motion} constraint. \textbf{Ours (full)} represents the full model with both \textit{content} and \textit{motion} refinement. The best results are highlighted.}
	\label{tab:ablation_study}
\end{table}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}

==> fig_tables/table_robotcar.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
%\setlength{\tabcolsep}{4.pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table}[t]
	\scriptsize
	%\footnotesize
	%\small
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{lcccc}
				\hline
				\hline
				& \multicolumn{4}{c}{Method} \\
				% \cline{2-15} 
				%Method & \multicolumn{2}{c}{03} & \multicolumn{2}{c}{04} & \multicolumn{2}{c}{05} & \multicolumn{2}{c}{06} & \multicolumn{2}{c}{07} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{Avg}\\ 
				Scene & Stereo VO \cite{robotcar2017} & PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric} & MapNet \cite{brahmbhatt2018mapnet} & Ours \\
				LOOP1 & 35.84m, $14.23^\circ$ & 28.81m, $19.62^\circ$ & \textbf{8.76}m, $3.46^\circ$ & 9.07m, $\mathbf{3.31}^\circ$  \\
				LOOP2 & 40.20m, $12.85^\circ$ &25.29m, $17.45^\circ$ & 9.84m, $3.96^\circ$ &\textbf{9.19}m, $\mathbf{3.53}^\circ$ \\
				FULL1 & 222.0m, $13.7^\circ$ &125.6m, $27.1^\circ$ &41.4m, $12.5^\circ$ &\textbf{31.65}m, $\mathbf{4.51}^\circ$ \\
				FULL2 & 222.0m, $13.7^\circ$ &131.06m, $26.05^\circ$ &59.30m, $14.81^\circ$ &\textbf{53.45}m, $\mathbf{8.60}^\circ$ \\
				Avg & 99.35m, $13.59^\circ$ & 59.90m, $21.39^\circ$ & 20.0m, $6.64^\circ$ & \textbf{17.58}m, $\mathbf{4.25}^\circ$ \\
				%Method & LOOP1 & LOOP2 & FULL & Avg \\
				
				%Stereo VO \cite{kendall2015posenet} & 35.84m, $14.23^\circ$ & 40.20m, $12.85^\circ$ & 222.0m, $13.7^\circ$ & 99.35m, $13.59^\circ$\\
				%PoseNet \cite{kendall2015posenet} & 28.81m, $19.62^\circ$ & 25.29m, $17.45^\circ$ & 125.6m, $27.1^\circ$ & 59.90m, $21.39^\circ$\\
				%MapNet \cite{kendall2015posenet} & 8.76m, $3.46^\circ$ & 9.84m, $3.96^\circ$ & 41.4m, $12.5^\circ$ & 20.0m, $6.64^\circ$\\
				%Ours \cite{kendall2015posenet} & 9.07m, $3.31^\circ$ & 9.19m, $3.53^\circ$ & 34.48m, $6.64^\circ$ & 17.58m, $4.25^\circ$\\
				
				\hline
				\hline
			\end{tabular}
		\end{center}
	
	\caption{Mean translation and rotation errors of Stereo VO, PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}, MapNet \cite{brahmbhatt2018mapnet} nad our method on RobotCar dataset \cite{robotcar2017}. Result of Stereo VO are from \cite{robotcar2017}. Results of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. The best results are highlighted.}
	\label{tab:error_robotcar}
\end{table}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}

==> fig_tables/table_robotcar_extend_ablation.tex <==
%We would be glad to respond to further questions and comments you may have.
%\tiny
\setlength{\tabcolsep}{5.pt}
%\setlength\LTleft{-1in}
%\setlength\LTright{-1in plus 1 fill}
\begin{table*}[t]
	%\scriptsize
	%\footnotesize
	%\small
	\setlength{\abovecaptionskip}{0pt}%    
	\setlength{\belowcaptionskip}{0pt}%
	\centering
		\begin{center}
			%\resizebox{\textwidth}{15mm}{
			\begin{tabular}{lccccc}
				\hline
				\hline
				& \multicolumn{5}{c}{Method} \\
				% \cline{2-15} 
				%Method & \multicolumn{2}{c}{03} & \multicolumn{2}{c}{04} & \multicolumn{2}{c}{05} & \multicolumn{2}{c}{06} & \multicolumn{2}{c}{07} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{Avg}\\ 
				Scene &  PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric} & MapNet \cite{brahmbhatt2018mapnet} & Ours (basic) & Ours (content) & Ours \\
				FULL3 & 125.6m, $27.1^\circ$ &41.4m, $12.5^\circ$ &\textbf{31.65}m, $\mathbf{4.51}^\circ$ & 41.4m, $12.5^\circ$&41.4m, $12.5^\circ$ \\
				FULL4 & 131.06m, $26.05^\circ$ &59.30m, $14.81^\circ$ &\textbf{53.45}m, $\mathbf{8.60}^\circ$ & 41.4m, $12.5^\circ$&41.4m, $12.5^\circ$\\
				FULL5 & 125.6m, $27.1^\circ$ &41.4m, $12.5^\circ$ &\textbf{31.65}m, $\mathbf{4.51}^\circ$  & 41.4m, $12.5^\circ$&41.4m, $12.5^\circ$\\
				FULL6 & 131.06m, $26.05^\circ$ &59.30m, $14.81^\circ$ &\textbf{53.45}m, $\mathbf{8.60}^\circ$ &41.4m, $12.5^\circ$ &41.4m, $12.5^\circ$\\
				FULL7 & 125.6m, $27.1^\circ$ &41.4m, $12.5^\circ$ &\textbf{31.65}m, $\mathbf{4.51}^\circ$ & 41.4m, $12.5^\circ$&41.4m, $12.5^\circ$ \\
				FULL8 & 131.06m, $26.05^\circ$ &59.30m, $14.81^\circ$ &\textbf{53.45}m, $\mathbf{8.60}^\circ$ & 41.4m, $12.5^\circ$&41.4m, $12.5^\circ$\\
				Avg & 77.85m, $22.56^\circ$ & 29.83m, $8.68^\circ$ & \textbf{25.84}m, $\mathbf{4.99}^\circ$ & 41.4m, $12.5^\circ$&41.4m, $12.5^\circ$\\
				
				\hline
				\hline
			\end{tabular}
		\end{center}
	
	\caption{Mean translation and rotation errors of PoseNet \cite{kendall2015posenet, kendall2016modelling, kendall2017geometric}, MapNet \cite{brahmbhatt2018mapnet} nad our method on Oxford RobotCar dataset \cite{robotcar2017}. Results of PoseNet and MapNet are from \cite{brahmbhatt2018mapnet}. The best results are highlighted.}
	\label{tab:error_robotcar_extend}
\end{table*}
%\setlength{\tabcolsep}{1.4pt}
%\setlength{\textfloatsep}{0cm}
